Impact of ionizing radiation on superconducting qubit coherence

The practical viability of any qubit technology stands on long coherence times and high-fidelity operations, with the superconducting qubit modality being a leading example. However, superconducting qubit coherence is impacted by broken Cooper pairs, referred to as quasiparticles, with a density that is empirically observed to be orders of magnitude greater than the value predicted for thermal equilibrium by the Bardeen-Cooper-Schrieffer (BCS) theory of superconductivity. Previous work has shown that infrared photons significantly increase the quasiparticle density, yet even in the best isolated systems, it still remains higher than expected, suggesting that another generation mechanism exists. In this Letter, we provide evidence that ionizing radiation from environmental radioactive materials and cosmic rays contributes to this observed difference, leading to an elevated quasiparticle density that would ultimately limit superconducting qubits of the type measured here to coherence times in the millisecond regime. We further demonstrate that introducing radiation shielding reduces the flux of ionizing radiation and positively correlates with increased coherence time. Albeit a small effect for today's qubits, reducing or otherwise mitigating the impact of ionizing radiation will be critical for realizing fault-tolerant superconducting quantum computers.

==> figure_captions.tex <==
\clearpage
\section*{Figure captions}
\subsection*{Figure 1}
{\bf Schematic of the experiment.} 
    %
    a) Illustration of the sample holder and the \ce{^64}{Cu} radiation source. The source is mounted \SI{3.3}{\milli\metre} above the silicon chip containing the superconducting aluminum transmon qubits. 
    %
    b) False-color micrograph and circuit schematic of the qubit sample. The sample consists of two transmon qubits, Q1 (blue, left) and Q2 (orange, right). The resonators used to readout the qubits are shown with red and cyan. The resonators are inductively coupled to a common microwave transmission line, through which both qubit control and readout pulses are sent. The control pulses and the measurement pulses are generated using microwave sources and arbitrary waveform generators at room temperature (not shown, see Extended Data Fig. \ref{fig:ex2}e). 
    %
    c) Diagram of the possible quasiparticle generation processes. Incoming ionizing radiation (from $\beta^{\pm}$, $\gamma$, and cosmic rays) interact with the Al qubit and Si substrate, creating electron-hole pairs due to the ionization of atoms and phonons (see text). The subsequent energy cascade of these particles ultimately breaks Cooper pairs and thereby generates quasiparticles.
\subsection*{Figure 2}
{\bf \ce{^64}{Cu} radiation exposure experiment.} 
    %
    a) Measured energy relaxation rates $\Gamma_1 = 1/T_1$ of qubits Q1 (blue) and Q2 (orange) as a function of time when exposed to the \ce{^64}{Cu} source. The inset shows an example of the raw data used for fitting the energy relaxation rates. Blue points are the median of 20 measured qubit excited-state populations $p(t)$ at various times after the excitation pulse. Blue bars indicate the 95\% confidence interval for the median. The orange line is the exponential fit to the data, given in Eq.~\eqref{eq:coherence}. 
    The super-exponential decay at short measurement times results from 
    %statistical fluctuation in the quasiparticle number and its impact on the %induced 
    statistical fluctuations in the quasiparticle-induced
    energy-relaxation rate during the 20 measurements~\cite{Gustavsson1573}.
    %
    b) Power density of the radiation during the experiment derived from radiation transport simulations (see text). 
    %
    c) Energy relaxation rates $\Gamma_1$ as a function of radiation power density. The solid lines show the fit to the model of Eq.~\eqref{eq:simple_qp_model}. The dashed lines show the fit to model of Eq.~\eqref{eq:simple_qp_model} with $\Gamma_{\rm other} = 0$ and $P_{\rm int} = 0$. The vertical red line is the radiation power density level due to the external radiation $P_{\rm ext}$.
\subsection*{Figure 3}
{\bf Environmental radioactivity assessment.} {a) Spectrum of $\gamma$-radiation in the laboratory measured with NaI scintillation detector, binned in 8192 energy bins. The data is fit to the weighted sum of simulated spectra from \ce{^238}{U},\ce{^232}{Th}, and \ce{^40}{K} progenitors convolved with a response function of the NaI detector. These isotopes are typical contaminants in concrete.
b) Simulated spectral density of power absorbed in the aluminum film that comprises the qubit, calculated with Geant4 using the measured spectrum shown in panel a) and the emission spectra of the \ce{^64}{Cu} source and its impurities. At $t=0$, the spectrum is dominated by \ce{^64}{Cu}, after 12 days by \ce{^198}{Au} impurities, and after 36 days by \ce{^{\rm 110m}}{Ag}. \ce{^32}{Si} is a radioactive contaminant intrinsic to the silicon substrate~\cite{Aguilar-Arevalo:2016ndq}. The fluctuations in the simulated spectra are due to finite simulation statistics.
\subsection*{Figure 4}
{\bf Qubit shielding experiment.} 
    %
    a) Schematic of shielding experiment. The qubit energy relaxation rate is measured $N$ times with the shield up, and then again $N$ times with the shield down. This cycle is repeated 65 times for qubits Q1 and Q2 and 85 times for qubits Q3-Q7.
    %a) shows the schematic of the shielding experiment. The energy relaxation rate of all the qubits is measured for 10 minutes after which the shield was lowered or raised. The red ellipses show the pairs of measurements which are compared in the A/B test. 
    %
    b) Histogram of the differences in energy relaxation rates when the shield is up versus down. The inset shows the histogram peak. The orange vertical line indicates the median of the distribution. Although the median difference in the relaxation rates between shield-up and shield-down configurations is only 1.8\% of the width of the distribution, it differs from zero in a statistically significant manner. 
    %
    c) Difference in the energy relaxation rates in the shielding experiment (orange dot) versus $P_{\rm int} / P_{\rm ext}$. Vertical error bars are the 95\% confidence intervals for the median of $\delta\Gamma_1$. Horizontal error bars are the corresponding confidence intervals for $P_{\rm int}$. The blue line indicates the energy relaxation rate estimated using the model from the \ce{^64}{Cu} radiation exposure measurement and Eq. \eqref{eq:delta_gamma}. The filled blue region shows the confidence interval for the estimate assuming $\pm$ 20\% relative error for $P_{\rm ext}$. Below the gray dashed line, the experiment is not sensitive enough to detect $\delta\Gamma_1$.

\subsection*{Extended Data Figure 1}
{\bf Experimental set-up.} {\bf a} The diagram shows a simplified block diagram of the room temperature electronics and dilution refrigerator configuration used for measuring the qubit frequency and coherence times. Panels {\bf b-d} show the schematic of the lead shield used to block environmental radiation. The lead shield can be raised and lowered using a scissor lift. {\bf b} In the up-position, the qubits were \SI{17}{\centi\metre} below the edge of the lead shield. {\bf c} In the lowered position the edge of the lead shield was \SI{120}{\centi\metre} below the qubits. {\bf d} Picture of a partially-raised lead shield [in between the configurations shown in panels {\bf b} and {\bf c}]. The lead bricks are wrapped in protective plastic film. {\bf e} The parameters of the qubits used in the lead shield experiment.

\subsection*{Extended Data Figure 2}
{\bf Quasiparticle injection experiment.} {\bf a} shows the pulse sequence in the quasiparticle injection experiment. First a strong microwave pulse is applied for the duration of $d_{\rm qp}$ to the resonator, which excites quasiparticles. After time $t_{\rm qp}$ the { energy-relaxation time} of the qubit is measured. {\bf b} shows the energy relaxation rate of the qubit Q1 during the quasiparticle injection experiment (blue dots). A solid green line shows a fit to the data using the full model that includes quasiparticle trapping and recombination. Orange dash dotted line shows the model with only recombination, dotted line shows the same model without the internal quasiparticle relaxation rate $\Gamma_{\rm other}$. Blue dash dotted line shows the fit to the model that only includes trapping of quasiparticles. Dotted blue line shows the trapping model without $\Gamma_{\rm other}$.

\subsection*{Extended Data Figure 3}
{\bf Energy-relaxation times in the shielding experiment}. Energy relaxation times $T_1$ for qubits Q1-Q7 during the lead shield experiment while the shield is in up (blue) or down (orange) positions. {\bf b} shows the pulse sequence used to measure the energy relaxation rate of all the qubits. First a $\pi$ pulse is applied to all the qubits. After time $t$ a measurement pulse is used to determine the state of the qubits. The qubit excited state population relaxes exponentially as a function of time. Blue circles show the measured qubit excited state populations and the orange line is an exponential fit using the model of Eq. \eqref{eq:gamma_1}. {\bf c} Stacked histogram of the combined energy relaxation times for all of the qubits in the lead shield experiment. {\bf d} Plot of the noise power spectral density during the lead shield experiment for qubits Q3, Q4, Q6, and Q7. The red dashed red line marks the rate of a single cycle of the lead shield. The green dashed line shows the estimated measurement period if all the data was gathered sequentially. Orange line is a fit to a power law $S = {\rm const}/f^\alpha$ with $\alpha \approx 1.5$.

\subsection*{Extended Data Figure 4}
\textbf{Resonator single-tone spectroscopy.} \textbf{a-d} show the transmission profile of resonator 1 as as a function of readout power and readout frequency at different times throughout the experiment. When exposed to a high level of radiation, the resonator frequency becomes unstable in the dispersive regime which is used for reading out the qubit. The resonator becomes more stable as the radiation source decays. \textbf{e} shows the change in the resonance frequency, $\Delta \omega_{\text{r}}$, due to radiation through out the experiment. We observe that the median $\Delta \omega_{\text{r}}$ follows an exponential decay with a half-life of $t_{1/2}= (21.74 \pm 2.8) \si{\hour}$. Furthermore, in \textbf{f} we see the full-width-half-max (FWHM) of the resonator also exponentially decay with a half-life of $t_{1/2}= (24.16 \pm 0.78) \si{\hour}$ until converging to the control value.

\subsection*{Extended Data Figure 5}
{\bf Qubit frequency shift.} {\bf a} The frequency of the qubit can be determined from a Fourier transform of a Ramsey measurement, shown in the panel at different times after installation of the \ce{^64}{Cu} source. We plot the inferred qubit frequency by offsetting the measured Fourier transform spectra by the frequency of the control pulses. The orange dashed lines show the shift in the average qubit frequency during the experiment. {\bf b} The pulse sequence used in a Ramsey measurement. First $\pi/2$-pulse prepares the qubit in a superposition state. The phase of the qubit state evoles during time $t$, after which a second $\pi/2$-pulse is applied before the measurement pulse. {\bf c-e} Ramsey oscillations and fit $T_2$ times are shown at \SI{152}{\hour}, \SI{212}{\hour} and \SI{340}{\hour} after installation of the \ce{^64}{Cu} source. The dashed lines in panel {\bf a} show the times at which the measurements are performed.

\subsection*{Extended Data Figure 6}
{\bf Radiation transport simulations.} {\bf a} Isotopes measured to be present in the sample ``A-Ref'' and the activity inferred for each in sample ``A'' as of May 24, 2019 at 4:00 PM Eastern time zone. {\bf b} Results from simulations of environmental radiation sources in the laboratory environment.  The background gamma flux is obtained by a fit to a measurement with a NaI scintillator (Fig.~\protect{\ref{fig:fig3}}a), simulating and measuring both with and without the lead shield in the ``up'' position. Cosmic rays were also measured and simulated for both shield-up and shield-down conditions; the shield did not have a measurable effect in the ``up'' position, as expected, and the effect is taken to be zero in the ``down'' position. {\bf c} The Average shield efficiency values for $\eta$ are weighted by each component's contribution to total external power. 
Statistical uncertainties on the fraction of flux reaching the interior of the DR are all 0.0001; uncertainties on $\eta$ values for individual isotopes are all approximately 0.001. {\bf d} Power densities absorbed in silicon and aluminum. {\bf e} The figure shows the spectrum of the energy deposited in a NaI detector by cosmic ray muon secondaries measured in the laboratory. Blue solid line shows the known cosmic ray muon spectrum fit to the measured data. The spectrum corresponding to energies below the dashed red line is shown in Fig. \ref{fig:fig3}a. Note that in the spectrum shown here a different energy bin width is used to capture higher energy scales.

\subsection*{Extended Data Figure 7}
{\bf The effect of post-processing on the lead shield effect A/B test.} {\bf a} The upper row shows the p-value of the Wilcoxon signed rank test for three different test cases and for the different post-processing parameters. On the horizontal axis the $T_1^{\rm cutoff}$ is varied. The vertical axis shows the effect of applying a cutoff to the difference in the energy relaxation rates when the shield status is changed. The first column shows the actual data. The middle column shows a reference experiment, where the energy relaxation rates are compared without moving the shield. The last column shows the data when the energy relaxation rate pairs are randomized. The lower row shows the median of the effect of the shield on the energy relaxation rate $\delta\Gamma_1$. {\bf b} The median of $\delta\Gamma_1$ along the dashed lines in {\bf a}. The filled area shows 68\% confidence intervals for the median.

\subsection*{Extended Data Figure 8}
{\bf Asymmetry parameter distribution.} The distribution of the asymmetry parameter $\langle A \rangle$ of the energy relaxation rates between the shield in up or down position.
